CataNet: Predicting remaining cataract surgery duration

Cataract surgery is a sight saving surgery that is performed over 10 million times each year around the world. With such a large demand, the ability to organize surgical wards and operating rooms efficiently is critical to delivery this therapy in routine clinical care. In this context, estimating the remaining surgical duration (RSD) during procedures is one way to help streamline patient throughput and workflows. To this end, we propose CataNet, a method for cataract surgeries that predicts in real time the RSD jointly with two influential elements: the surgeon's experience, and the current phase of the surgery. We compare CataNet to state-of-the-art RSD estimation methods, showing that it outperforms them even when phase and experience are not considered. We investigate this improvement and show that a significant contributor is the way we integrate the elapsed time into CataNet's feature extractor.

==> Changes_after_review.tex <==
All changes are marked in the .tex document under \review{}
The following is a summary of them:

- Explained why we predict the experience level on every frame
- Explained why we show results for senior and assistant surgeons individually
- Added experiment on real-time capabilities of the model
- Added remaining challenges and future work
- Clarified further how the elapsed time was integrated into the model
- Clarified how we chose the minimum video length
- Explained how the baselines were selected
- Corrected how we perform stratified sampling
- Explained why we did not perform a leave-one-out experiment to test the experience performance

==> detailed-rsd.tex <==
In 2008, Padoy et al. \cite{Padoy2008} used Hidden Markov models (HMMs) for intervention time prediction based on high-level tasks. This was sort of an after-thought of their model and not really the main goal.
 
Surgical workflow management in the OR requires process information about the current surgical procedure \cite{Neumuth2012},
In \cite{Neumuth2012}, Neumuth et al. introduce a surgical workflow management system for to provide a robust guidance for surgical activities. Additionally they test it on cataract surgery, showing that for their dataset of 100 surgeries, 10\% of the procedures are sufficient to guide approximately 65\% of all surgical processes, and that 50\% are sufficient to guide approx. 80\% of all processes. 

In 2013, \cite{Franke2013}, Franke et al. present a model for remaining surgical time prediction and evaluate it's accuracy for two different neurosurgical interventions: discectomy and brain tumor resections.
Franke et al. proposed a system to predict intervention time from low-level surgical activities.

In 2016, Achiron et al.\cite{Achiron2016} show that there is a correlation between the patient's preoperative risk and the total length of the surgery. In this way, they train a system to predict the length of the surgery given a preoperative risk assessment. One star. Falls too strongly onto previous work.

In 2016, \cite{Guedon2016} used support vector machines to predict in real-time remaining procedure duration based on the activation pattern of one single piece of equipment, the electrosurgical device. They tested their system on 21 laparoscopic cholecystectomies, showing an improvement in accuracy over the estimations made by the OR staff.

In 2017, \cite{Spangenberg2017} utilized surgical phase events recognized in surgical device data to learn prediction models (regression) and trigger online predictions for remaining intervention times in operating rooms. That is, they are not using the data directly, but information such as: event name, even timestamp, operating room, surgeon, window length and opscode. They tested linear regression, decision tree regression, random forest regression and multilayer perceptron.

In 2017, Aksamentov et al.\cite{Aksamentov2017} propose automatic methods to estimate the remaining surgery duration in real-time by using only the image feed from the endoscopic camera and no other sensor. These approaches are based on neural networks designed to learn the workflow of an endoscopic procedure. 

In 2017, Maktabi and Neumuth~\cite{Maktabi2017}

In 2019, Twinanda et al.\cite{Twinanda2019} introduce RSDNet: Learning to predict remaining surgery duration from laparoscopic videos without manual annotations.
Also in 2019, Bodenstedt et al. \cite{Bodenstedt2019} propose and compare methods, based on convolutional neural networks, for continuously predicting the duration of laparoscopic interventions based on unlabeled data, such as from endoscopic image and surgical device streams.

Check also \cite{Rivoir2019}: present unsupervised temporal video segmentation as a novel auxiliary task for video-based remaining surgery duration (RSD) prediction and propose three different learning pipelines to
utilize unsupervised temporal segmentation learning for RSD modeling

""As indicated in \cite{Aksamentov2017,Twinanda2019}, progress-related features can be beneficial for RSD prediction. Using an unsupervised auxiliary task makes this approach widely applicable to different datasets."

==> oldstuffIamtooweaktojusterase.tex <==


\begin{table}[]
    \centering
    \begin{tabular}{lccc}
    \hline
                 &  (3) RSD  & (4) RSD no et & (5) RSD et after LSTM\\
                 \hline
    RSD  &  $1.11 \pm 0.62$ & $1.28 \pm 0.69$ & $1.34 \pm 0.73$ \\
    RSD-5 & $0.76 \pm 0.41$ & $0.92 \pm 0.58$ & $0.74 \pm 0.34$ \\
    RSD-2 & $0.39 \pm 0.28$ & $0.49 \pm 0.31$ & $0.44 \pm 0.20$ \\
    RSD@Hyd & $1.99 \pm 1.38$ & $1.99 \pm 1.10$ & $2.28 \pm 1.34$ \\
    \hline
    \end{tabular}
    \caption{RSD is the macro mean absolute error RSD throughout the surgery. RSD-2 is average of the last 2 mins. RSD-5 is average of the last 5 mins. RSD@2 is average at the second minute mark. All values are mean $\pm$ standard deviation in minutes.}
    \label{tab:rsdnetcomparison}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
    \hline
            & Densenet-full & Resnet-full     & Dense-noet & Resnet-noet \\
                 \hline
    RSD     & $0.99 \pm 0.65$   & $1.04 \pm 0.68$   & $1.28 \pm 0.69$ & $1.19 \pm 0.60$ \\
    RSD-5   & $0.64 \pm 0.56$   & $0.71 \pm 0.47$   & $0.92 \pm 0.58$ & $0.87 \pm 0.40$ \\
    RSD-2   & $0.35 \pm 0.20$   & $0.35 \pm 0.20$   & $0.49 \pm 0.31$ & $0.45 \pm 0.18$ \\
    RSD@Hyd & $1.66 \pm 1.35$   & $1.67 \pm 1.30$   & $1.66 \pm 1.35$ & $1.91 \pm 1.15$ \\
    \hline
    \end{tabular}
    \caption{RSD is the macro mean absolute error RSD throughout the surgery. RSD-2 is average of the last 2 mins. RSD-5 is average of the last 5 mins. RSD@Hyd is average at the end of hydrodissection step. All values are mean $\pm$ standard deviation in minutes.}
    \label{tab:trainingold}
\end{table}




\begin{table}[]
    \centering
    \begin{tabular}{lcc}
    \hline
            & RSDNet & RSDNet our training  \\
                 \hline
    RSD     & $1.59 \pm 0.69$   & $1.44 \pm 0.52$  \\
    RSD-5   & $1.37 \pm 0.83$   & $1.05 \pm 0.40$  \\
    RSD-2   & $1.23 \pm 0.53$   & $1.04 \pm 0.34$  \\
    RSD@Hyd & $2.32 \pm 1.27$   & $2.09 \pm 1.20$  \\
    \hline
    \end{tabular}
    \caption{RSD is the macro mean absolute error RSD throughout the surgery. RSD-2 is average of the last 2 mins. RSD-5 is average of the last 5 mins. RSD@Hyd is average at the end of hydrodissection step. All values are mean $\pm$ standard deviation in minutes.}
    \label{tab:trainingold}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{lccccccc}
    \hline
                 &  Complete  &  (1) step & (2) Exp & (3) RSD  & (4) no elapsed time & (5) prog no et\\
                 \hline
    MAE  &  $0.99 \pm 0.65$  & $0.98 \pm 0.58$  & $1.22 \pm 0.92$ & $1.11 \pm 0.62$ & $1.28 \pm 0.69$ & $1.26 \pm 0.71$ \\
    MAE-5 & $0.64 \pm 0.46$ & $0.74 \pm 0.56$ & $0.87 \pm 0.62$& $0.76 \pm 0.41$ & $0.92 \pm 0.58$ & $0.91 \pm 0.55$ \\
    MAE-2 & $0.35 \pm 0.20$ & $0.35 \pm 0.23$ & $0.51 \pm 0.27$& $0.39 \pm 0.28$ & $0.49 \pm 0.31$ & $0.49 \pm 0.29$ \\
    MAE@Hyd & $1.66 \pm 1.35$ & $1.43 \pm 1.19$ & $1.82 \pm 1.63$& $1.99 \pm 1.38$ & $1.99 \pm 1.10$ & $1.93 \pm 1.30$ \\
    \hline
    \end{tabular}
    \caption{RSD is the macro mean absolute error RSD throughout the surgery. RSD-2 is average of the last 2 mins. RSD-5 is average of the last 5 mins. RSD@2 is average at the second minute mark. All values are mean $\pm$ standard deviation in minutes.}
    \label{tab:ablation}
\end{table}

==> semi-supervised-learning.tex <==
In \cite{chen20j}, Chen et al. introduce SimCLR: a simple framework for contrastive learning of visual representations. They show that a linear classifier trained on self-supervised representations learned by SimCLR achieves the classification performance performance of a supervised ResNet-50.

In \cite{Han20}, Han et al. introduce MemDPC: Memory-augmented Dense Predictive Coding for Video Representation Learning. They show that it is possible to learn high-quality video representations with self-supervised learning, from the visual stream alone (without additional audio or text streams).
